Edge-Colored Clustering in Hypergraphs: Beyond Minimizing Unsatisfied Edges

We consider a framework for clustering edge-colored hypergraphs, where the goal is to cluster (equivalently, to color) objects based on the primary type of multiway interactions they participate in. One well-studied objective is to color nodes to minimize the number of unsatisfied hyperedges -- those containing one or more nodes whose color does not match the hyperedge color. We motivate and present advances for several directions that extend beyond this minimization problem. We first provide new algorithms for maximizing satisfied edges, which is the same at optimality but is much more challenging to approximate, with all prior work restricted to graphs. We develop the first approximation algorithm for hypergraphs, and then refine it to improve the best-known approximation factor for graphs. We then introduce new objective functions that incorporate notions of balance and fairness, and provide new hardness results, approximations, and fixed-parameter tractability results.

==> sections/graphmaxecc.tex <==
\begin{algorithm}[t]
	\caption{An approximation algorithm for \maxecc{}}
	\label{alg:graph_max_ecc}
	\begin{algorithmic}
		\STATE Obtain optimal LP variables $\{z_e; x_v^c\}$ for the relaxation
		\STATE $\pi \leftarrow \text{uniform random ordering of colors } [k]$
		% \FOR{$c \in [k]$}
		%     \STATE $\alpha_c \leftarrow \text{ a uniform random value in } [0, 1]$
		% \ENDFOR
		\STATE For $c \in [k]$, $\alpha_c \leftarrow $ uniform random threshold in $[0,1]$
		\FOR{$v \in V$}
		\STATE $S_v \leftarrow \left\{c \in [k] \mid x_v^c \geq 2/3 \right\}$; $W_v \leftarrow [k] \setminus S_v$
		% \STATE
		\STATE $W'_v = \left\{ c \in W_v \mid \alpha_c < x_v^c \right\}$
		% \STATE
		\IF{$|W'_v| > 0$}
		\STATE $\lambda(v) \leftarrow \argmax_{i \in W'_v} \pi(i)$
		\ELSIF{$\exists c \text{ s.t. } S_v = \left\{ c \right\}$}
		\STATE $\lambda(v) \leftarrow c$
		\ELSE
		\STATE $\lambda(v) \leftarrow \text{ arbitrary color}$
		\ENDIF
		\ENDFOR
	\end{algorithmic}
\end{algorithm}
Algorithm \ref{alg:graph_max_ecc} is our refined algorithm for \maxecc{} in graphs ($r = 2$). It solves the LP relaxation, generates color thresholds $\{\alpha_i \colon i \in [k]\}$, and generates a uniform random color permutation $\pi$ in the same way as Algorithm~\ref{alg:hyper_maxecc}. However, it differs in that it partitions colors for each $v$ into colors that $v$ wants \emph{strongly} or \emph{weakly}, given respectively by the sets:
\begin{align*}
	S_v = \{ i \in [k] \colon x_v^i \geq 2/3\} \text{ and } W_v &= [k] - S_v.
\end{align*}
The LP constraint $\sum_{i = 1}^k x_v^i = 1$ implies that $S_v$ can contain at most one color. It is also possible that $S_v = \varnothing$. We say color $i$ is \textit{strong for $v$} if $S_v = \{i\}$, otherwise $i$ \textit{weak for $v$}.

As a slight variation on our hypergraph algorithm, Algorithm~\ref{alg:graph_max_ecc} first checks if $v$ specifically wants any \emph{weak} colors (as determined by color thresholds $\{\alpha_c \colon c \in [k]\}$. If so, it gives $v$ the weak color with highest priority (as defined by $\pi$). If $v$ wants to weak colors but has a strong color, then $v$ is assigned the strong color. If neither happens, $v$ is given an arbitrary color. 
%
Prioritizing weak colors in this way appears counterintuitive, since if $v$ has a strong color it is a strong indication that $v$ should be color $c$. To explain the rationale: note that $x_v^c \geq 2/3$ still implies $v$ will be given color $c$ with high probability, since a large value for $x_v^c$ makes it less likely $v$ will want other colors. Meanwhile, prioritizing other colors will make it possible to lower bound the probability that an edge $e = (u,v)$ is satisfied even if $\ell(e)$ is not strong for $u$ or $v$.
Concretely, we are able to prove the following result for an arbitrary edge $e$, which proves our approximation guarantee.
\begin{theorem}
	\label{thm:graphecc}
	For every $e \in E$, $\prob[\text{$e$ is satisfied}] \geq p z_e$ where $p = \frac{154}{405} > 0.38$ when running Algorithm~\ref{alg:graph_max_ecc}.
\end{theorem}
To prove this result, we fix $e = (u,v)$ with color $c = \ell(e)$ and set $C = [k] \backslash \{c\}$. As before, $X_v^i$ is the event that $v$ wants color $i$. We furthermore use $Y_v^i$ to denote the event that $v$ is \emph{actually assigned} color $i$ by Algorithm~\ref{alg:graph_max_ecc}. We define $N_v$ to be the event that $v$ wants \emph{no} colors in $C$. If $c$ is strong for $v$, the event $N_v$ is equivalent to the event that $v$ wants no weak colors and is therefore assigned color $c$. Events $X_u^i$, $Y_u^i$, and $N_u$ are defined analogously for u. Our proof of Theorem~\ref{thm:graphecc} relies on the following supporting lemma.
% some of which are purely algebraic that are independent of ECC, and some of which directly use our notation four our LP rounding techniques. 
\begin{lemma}
	\label{lem:dependent_y_n_x}
	Given an edge $e = (u,v)$ of color $c$ {with \color{blue} $S_v = \{c\}$, and $c \in W_u$,} we have
	\[
	\prob\left[Y_u^c \mid N_v \cap X_u^c\right] \geq \prob\left[Y_u^c \mid X_u^c\right].
	\]
\end{lemma}
We also require the following definition and Lemmas~\ref{lem:sum_to_prod}-\ref{lem:bounding_constraints}, which are purely algebraic but will be used at various points to bound certain probabilities. 

For intuition, if we consider a set of $m$ mutually independent events $\mathcal{E} = \{E_1, E_2, \cdots, E_m\}$, whose probabilities are encoded in a vector $\vx$ where the $i$th entry is $x_i = \prob[E_i]$, the function $P$ in Definition~\ref{def:prob} is the probability that exactly $t$ of the events in $\mathcal{E}$ happen. In practice, we will apply this with $\mathcal{E}$ representing a subset of colors in the ECC instance, and the vector $\vx$ encoding LP variables for some node $u$ and that set of colors (which by Observation~\ref{obs:cv} are probabilities for wanting those colors). Lemmas~\ref{lem:bounding} and \ref{lem:bounding_constraints} will then aid in bounding the probability that a node is assigned a certain color, conditioned on how many other colors it wants. 

\begin{definition}
	\label{def:prob}
	Let $m$ be a nonnegative integer and $t$ be an integer. Given a vector $\vx \in \mathbb{R}^m$, if $m \geq t > 0$, we define the function $P(\vx, t)$ as follows:
	\[
	P(\vx, t) = \sum_{I \in {[m] \choose t}} \left( \prod_{i \in I} x_i \prod_{j\in [m] \setminus I} (1 - x_j) \right),
	\]
	and for other choices of $t$ and $m$ we define
	\begin{equation*}
		P(\vx, t) = \begin{cases}
			0 & \text{ if $m < t$ or $t < 0$} \\
%			0 & \text{ if $t < 0$} \\
			1 & \text{ if $0 = m = t$} \\
			\prod_{i = 1}^m (1 - x_i) & \text{ if $0 = t < m$.}
		\end{cases} 
	\end{equation*}
\end{definition}

\begin{lemma}
	\label{lem:sum_to_prod}
	Let $\beta \in [0,1]$ be a constant and $\mathbf{x} \in \mathbb{R}^m_{\geq 0}$ be a length $m$ nonnegative vector satisfying $\sum_{t=1}^m x_t \leq \beta$, then we have $\prod_{t=1}^m (1 - x_t) \geq 1 - \beta$.
\end{lemma}

\begin{lemma}
	\label{lem:bounding}
	Let $m \geq 2$ be an integer and
	$a_0, a_1, \hdots, a_m$ be values such that for every $t \in [0, m-2]$, $a_{t+1} \leq a_t$ and $2 a_{t+1} \leq a_t + a_{t+2}$.
	Let $\mathcal{D} = \{ \vx \in [0,2/3]^m \colon \sum_{i = 1}^m x_i \leq 1 \}$ be the domain of a function
	$f : \mathcal{D} \rightarrow \mathbb{R}$ defined as
	\[
	f(\vx) = \sum_{t=0}^m a_t P(\vx, t).
	\]
	Then $f$ is minimized (over domain $\mathcal{D}$) by any vector $\vx^*$ with one entry set to $2/3$, one entry to $1/3$, and every other entry to $0$. Furthermore we have
	\begin{equation}
		\label{eq:minval}
		f(\vx^*) = \frac{2}{9}(a_0 + a_2) + \frac{5}{9}a_1.
	\end{equation}
\end{lemma}
The following lemma shows two choices for the sequence $\{a_t\}$ for which the conditions in Lemma \ref{lem:bounding} hold.
\begin{lemma}
	\label{lem:bounding_constraints}
	The inequalities $a_t \geq a_{t+1}$ and $a_t + a_{t+2} \geq 2 a_{t+1}$ hold for sequence $a_t = \frac{1}{1+g+t}$ where $g \geq 0$ is an arbitrary fixed integer. These inequalities also hold for the sequence
	\begin{align*}
		a_t &= \frac{2}{9}\left( \frac{1}{t+1} + \frac{1}{t+3} \right) + \frac{5}{9} \left( \frac{1}{t+2} \right).
	\end{align*}
\end{lemma}
\begin{proof}[Proof of Theorem~\ref{thm:graphecc}]
	
	We break the proof up into three cases, which depend on whether 2, 1, or neither of the nodes in $e = (u,v)$ have $c = \ell(e)$ as a strong color.
	
	\textbf{Case 1:} $c$ is strong for both $u$ and $v$, i.e., $S_u = S_v = \{c\}$.\\
	Since $c$ is the strong color for both $u$ and $v$, $e$ is satisfied if and only if $W'_u = W'_v = \emptyset$. Additionally, because nodes can only have a single strong color and we know $c$ is strong for both $u$ and $v$ we know that all other colors must be weak for both $u$ and $v$. Using the property that probabilities regarding separate colors are independent we have
	\begin{align*}
		\prob\left[e \text{ is satisfied}\right] & = \prob\left[W'_u = W'_v = \emptyset\right] \\
		& = \prod_{i \in C}\prob\left[ i \notin W'_u \cup W'_v \right]
	\end{align*}
	Consider a color $i \in C_v$, which by definition means $x_v^i \geq x_u^i$. There are three options for the random threshold $\alpha_i$:
	\begin{itemize}
		\item $\alpha_i < x_u^i \leq x_v^i$, which happens with probability $x_u^i$ and implies that $i \in W'_u \cap W'_v$,
		\item $x_u^i < \alpha_i \leq x_v^i$, which happens with probability $x_v^i - x_u^i$ and implies $i \in W'_v$, $i \notin W'_u$, and
		\item $x_u^i \leq x_v^i < \alpha_i$, which happens with probability $1 - x_v^i$ and implies $i \notin W_u' \cup W_v'$.
	\end{itemize}
	Thus, for $i \in C_v$ we have $\prob\left[i \notin W'_u \cup W'_v\right] = (1 - x_v^i)$ and similarly for $i \in C_u$ we have $\prob\left[i \notin W'_u \cup W'_v\right] = (1 - x_u^i)$. This gives
	\begin{align*}
		\prod_{i \in C}\prob\left[ i \notin W'_u \cup W'_v \right] & = \prod_{i \in C_v}(1 - x_v^i)\prod_{i \in C_u}(1 - x_u^i).
	\end{align*}
	The fact that $c$ is strong for both $u$ and $v$ means $x_v^i \geq 2/3$ and $x_u^i \geq 2/3$. From the equality constraint in the LP we see that for $w\in\{u,v\}$ we have $\sum_{i \in C}x_w^i \leq 1 - 2/3 = 1/3$. Applying Lemma \ref{lem:sum_to_prod} gives
	\begin{align*}
		\prod_{i \in C_v}(1 - x_v^i)\prod_{i \in C_u}(1 - x_u^i) & \geq \frac{2}{3}\frac{2}{3} = \frac{4}{9} \geq \frac{4}{9}z_e.
	\end{align*}

	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\textbf{Case 2:} $c$ is strong for one of $u$ or $v$. \\
	Without loss of generality we say $S_v = \{c\}$ and $c \in W_u$. 
	Edge $e$ is satisfied if and only if $Y_u^c \cap Y_v^c$ holds. 
	Because $c$ is strong for $v$, event $Y_v^c$ holds if and only if $N_v$ holds. Using the fact that $Y_u^c = Y_u^c \cap X_u^c$, we can write
	\[
	\prob\left[e \text{ is satisfied}\right] = \prob\left[Y_u^c \cap X_u^c \cap N_v\right].
	\]
	Using Bayes' Theorm, the fact that $X_u^c$ and $N_v$ are independent\footnote{Independence follows from the fact that $X_u^c$ is concerned with color $c$, while $N_v$ is concerned with a disjoint color set $C = [k]\backslash \{c\}$.}, Observation~\ref{obs:cv}, and Lemma~\ref{lem:dependent_y_n_x}, we see that
	\begin{align*}
		\prob\left[Y_u^c \cap X_u^c \cap N_v\right] & = \prob\left[ Y_u^c \mid N_v \cap X_u^c \right] \prob\left[ N_v \cap X_u^c \right] \\
		& = \prob\left[ Y_u^c \mid N_v \cap X_u^c \right] \prob\left[ N_v \right] \prob\left[ X_u^c \right] \\
		& = \prob\left[ Y_u^c \mid N_v \cap X_u^c \right] \prob\left[ N_v \right] x_u^c \\
		& \geq \prob\left[ Y_u^c \mid N_v \cap X_u^c \right] \prob\left[ N_v \right] z_e \\
		& \geq \prob\left[ Y_u^c \mid X_u^c \right] \prob\left[ N_v \right] z_e.
	\end{align*}
	Lemma \ref{lem:dependent_y_n_x} then gives
	\begin{align*}
		\prob\left[ Y_u^c \mid N_v \cap X_u^c \right] \prob\left[ N_v \right] z_e & \geq \prob\left[ Y_u^c \mid X_u^c \right] \prob\left[ N_v \right].
	\end{align*}
	Using $\overline{X}_v^i$ to indicate $v$ \emph{does not} want $i$, we get
	\[
	\prob\left[ N_v \right] = \prob\left[ \bigcap_{i \in C} \overline{X}_v^i \right] = \prod_{i \in C}(1 - x_v^i).
	\]
	As in Case 1, because $c$ is strong for $v$, we know that $\sum_{i \in C} x_v^i \leq 1/3$ and applying Lemma \ref{lem:sum_to_prod} gives us that $\prob\left[ N_v \right] \geq 2/3$. 
	
	
	Finally we must bound $\prob\left[ Y_u^c \mid X_u^c \right]$. Since 
	$c$ is weak for $u$ (i.e., $c \in W_u$), it will be convenient to consider all weak colors for $u$ other than $c$, which we will denote by $\hat{W}_u = W_u \backslash \{c\}$. We will then use $\hat{W}_u' = \{ i \in \hat{W}_u \colon \alpha_i < x_u^i\}$ to denote the set of colors in $\hat{W}_u$ that $u$ wants. Note that $X_u^c$ is independent of the number of colors in $\hat{W}_u$ that $u$ wants. 
	
	Because of the global ordering of colors, conditioned on $u$ wanting $c$ and wanting exactly $t$ colors in $\hat{W}_u$, there is a $1/(t+1)$ chance that $c$ is chosen first by the permutation $\pi$, and is therefore assigned to $u$. Formally:
	\begin{equation*}
		\prob\left[ Y_u^c \mid X_u^c  \cap (|\hat{W}'_u| = t)\right] = \frac{1}{t+1}.
	\end{equation*}
	We define $p_t = \prob[ |\hat{W}'_u| = t]$, that is the probability that exactly $t$ colors from $\hat{W}_u$ are wanted. Using the vector $\vx_v[\hat{W}_u]$ to encode LP variables for node $v$ for the colors in $\hat{W}_u$ we see that $p_i = P(\vx_v[\hat{W}_u], i)$. Therefore, the law of total probability implies
	\begin{equation}
		\label{eq:mainprob}
		\prob\left[ Y_u^c \mid X_u^c \right] 
		% = p_0 + \frac{1}{2}p_1 + \cdots + \frac{1}{|\hat{W}_u| + 1}p_{|\hat{W}_u|}.
		= \sum_{t = 0}^{|\hat{W}_u|} \frac{1}{1+t} p_t.
	\end{equation}
	Eq.~\eqref{eq:mainprob} is exactly of the form in Lemma \ref{lem:bounding} with $a_t = 1/(t+1)$. From Lemma \ref{lem:bounding_constraints}, we know this sequence $\{a_t\}$ satisfies the constraints needed by Lemma \ref{lem:bounding}. Combining this with the bound established earlier on $\prob\left[ N_v \right]$ gives
	\begin{align*}
		\prob\left[e \text{ is satisfied}\right] & \geq \prob\left[ Y_u^c \mid X_u^c \right] \prob\left[ N_v \right] z_e \\
		& \geq \frac{31}{54} \cdot \frac{2}{3} z_e = \frac{31}{81}z_e > 0.3827 z_e.
	\end{align*}

	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\textbf{Case 3:} $c$ is weak for both $u$ and $v$, i.e., $c \in W_u \cap W_v$.\\
	First we condition the probability of satisfying $e$ on the event $X_u^c \cap X_v^c$. If one of $X_u^c$ or $X_v^c$ does not happen, then $e$ cannot be satisfied, so we have
	\begin{align*}
		\prob\left[ \text{$e$ is satisfied} \right]&= \prob\left[ \text{$e$ is satisfied} \mid X_u^c \cap X_v^c \right] \prob\left[ X_v^c \cap X_u^c \right] \\
		&= \prob\left[ \text{$e$ is satisfied} \mid X_u^c \cap X_v^c \right] z_e.
	\end{align*}
	Define $D = (W_u \cup W_v) \backslash \{c\}$ to be the set of weak colors (excluding $c$) that want at least one of $\{u,v\}$. If we condition on $u$ and $v$ both wanting $c$, it is still possible that $e$ will not be satisfied because a weak color $i \in D$ wants either $u$ or $v$, and the permutation $\pi$ will prioritize color $i$ over $c$. We bound the probability of satisfying $e$ by conditioning on the number of such colors in $D$ that end up being wanted. 
	
	Using the same logic as in Observation~\ref{obs:cv}, we can present a simpler way to characterize whether a color $i \in D$ wants at least one of $\{u,v\}$. Formally, we partition $D$ into the sets:
	\begin{align*}
		D_u &= \{i \in D \colon x_u^i \geq x_v^i \} \\
		D_v &= D - D_v.
	\end{align*}
	Note that a color $i \in D_u$ wants one or both nodes in $e$ if and only if $i$ wants $u$, and color $i \in D_v$ wants one or both nodes in $e$ if and only if $i$ wants $v$.  
	Mirroring our previous notation, let $D_u'$ denote the set of colors in $D_u$ that want node $u$ (based on the random color thresholds) and define $D_v'$ analogously. The set $D_u' \cup D_v'$ is then the set of weak colors that want one or more node in $e$. Thus, conditioned on $|D_u' \cup D_v'| = t$ and conditioned on $u$ and $v$ wanting $c$, in order for $e$ to be satisfied $c$ must come before all $t$ colors in $|D_u' \cup D_v'|$ in the random permutation $\pi$. Formally, this means
	\[
	\prob\left[ \text{$e$ is satisfied} \mid X_u^c \cap X_v^c \cap (|D'_u \cup D'_v| = t) \right] = \frac{1}{1 + t}.
	\]
	
	Again using the law of total probability and the fact that $X_u^c \cap X_v^c$ is independent from the size of $D_u' \cup D_v'$, we see
	\begin{align}
		\label{eq:dupdvp}
		\prob[ e &\text{ is satisfied} \mid X_u^c \cap X_v^c ]
		= \sum_{t = 0}^{|D|} \frac{1}{1+t} \prob\left[ |D'_u \cup D'_v| = t \right].
	\end{align}
	
	Observe now that $D_u$ and $D_v$ are disjoint color sets, which implies that $|D_u'|$ and $|D_v'|$ are independent random variables. This allows us to decouple $D_u'$ and $D_v'$ in the above expression since $\prob\left[ |D'_u \cup D'_v| = t \right] = \prob\left[ |D'_u| + |D'_v| = t \right]$. We define 
	\[
	p_i = \prob\left[ |D'_u| = i \right] \text{ and } q_i = \prob\left[ |D'_v| = i \right],
	\] 
	so that we can write
	\[
	\prob\left[ |D'_u| + |D'_v| = t \right] = \sum_{\substack{i, j \in [0, t] \\ i + j = t}} p_i q_j = \sum_{i = 0}^{|D_u|} p_i q_{t-i} .
	\]
	This allows us to re-write Eq.~\eqref{eq:dupdvp} as follows:
	\begin{align}
		\label{eq:decoupled}
		\prob[ e \text{ is satisfied} \mid X_u^c \cap X_v^c ] &= \sum_{i = 0}^{|D_u|} \sum_{j = 0}^{|D_v|} \frac{1}{1+i+j} p_i q_j.
	\end{align}
	
	Without loss of generality we now assume $|D_u| \leq |D_v|$. We now proceed case by case depending on the sizes of $D_u$ and $D_v$. As a shorthand we use $\rho = \prob[ e \text{ is satisfied} \mid X_u^c \cap X_v^c ]$. Our goal is to show $\rho \geq 154/405$. In the cases below, we use the vector $\vx_u[D_u]$ to encode LP variables for node $u$ and colors in $D_u$ so that $p_i = P(\vx_u[D_u], i)$, and likewise $q_i = P(\vx_v[D_v], i)$, to match with notation in Definition~\ref{def:prob} and Lemma~\ref{lem:bounding}.
	
	\textbf{Case 3a.} $|D_u| = |D_v| = 0$. \\
	No weak colors other than $c$ want $u$ or $v$, so $\rho = 1$.
	
	\textbf{Case 3b.} $|D_u| = 0$ and $|D_v| = 1$. \\
	Letting $a$ be the single color in $D_v$,
	\begin{align*}
		\rho & = p_0 q_0 + \frac{1}{2} p_0 q_1 = q_0 + \frac{1}{2} q_1 = (1 - x_v^a) + \frac{1}{2} x_v^a.
	\end{align*}
	Because $a$ is a weak color for $v$, we know $x_v^a \in [0, \frac{2}{3}]$, and the minimum value the probability can obtain is $\frac{2}{3} > \frac{154}{405}$.
	
	
	\textbf{Case 3c.} $|D_u| = |D_v| = 1$. \\
	Letting $a$ be the color in $D_v$ and $b$ be the color in $D_u$,
	\begin{align*}
		\rho & = p_0 q_0 + \frac{1}{2}(p_0 q_1 + p_1 q_0) + \frac{1}{3} p_1 q_1 \\
		& = (1 - x_u^b)(1 - x_v^a) \\ & ~~~~~~~~~~+ \frac{1}{2}((1 - x_u^b)x_v^a + x_u^b(1 - x_v^a)) + \frac{1}{3} x_u^b x_v^a.
	\end{align*}
	Because $a$ is weak for $v$ and $b$ is weak for $u$, we know $x_v^a, x_u^b \in [0, \frac{2}{3}]$. This gives a minimum value for the probability of $\frac{13}{27} > \frac{154}{405}$. 
	
	\textbf{Case 3d.} $|D_u| = 0$ and $|D_v| > 1$. \\
	In this case $p_0 = 1$, and Eq.~\eqref{eq:decoupled} simplifies to
	\begin{equation*}
		\rho = \sum_{j = 0}^{|D_v|} \frac{1}{j+1} q_j \geq \frac{31}{54},
	\end{equation*}
	where we have applied Lemma \ref{lem:bounding} with $a_j = \frac{1}{j+1}$.
	
	\textbf{Case 3e.} $|D_u| = 1$ and $|D_v| > 1$. \\
	Eq.~\eqref{eq:decoupled} simplifies to
	\begin{align*}
		\rho &= p_0 \sum_{j = 0}^{|D_v|} \frac{q_j}{j+1}  + p_1 \sum_{j = 0}^{|D_v|} \frac{q_j}{j+2} \geq p_0 \frac{31}{54} + p_1 \frac{19}{54},
	\end{align*}
	where we applied Lemma \ref{lem:bounding} twice, once with $a_j = \frac{1}{j+1}$ and once with $a_j = \frac{1}{j+2}$. The right hand side of the above bound has a minium value of $\frac{23}{54}$.
	
	\textbf{Case 3f.} $|D_u| > 1$ and $|D_v| > 1$.
	From Eq.~\eqref{eq:decoupled} we know
	\begin{align*}
		\rho &= \sum_{i = 0}^{|D_u|}  p_i \left(\sum_{j = 0}^{|D_v|} \frac{1}{1+i+j}  q_j \right).
	\end{align*}
	We then apply Lemma~\ref{lem:bounding} $|D_v|$ times, where the $i$th time we apply it we use $a_j = \frac{1}{1+i+j}$. 
	which yields the bound
	\begin{align}
		\label{eq:lemdvtimes}
		\sum_{j = 0}^{|D_v|} \frac{1}{1+i+j}  q_j \geq \frac{2}{9}\left( \frac{1}{i+1} + \frac{1}{i+3} \right) + \frac{5}{9} \left( \frac{1}{i+2} \right).
	\end{align}
	The right hand of~\eqref{eq:lemdvtimes} defines a new sequence
	\begin{equation}
		\label{eq:uglyai}
		a_i = \left( \frac{1}{i+1} + \frac{1}{i+3} \right) + \frac{5}{9} \left( \frac{1}{i+2} \right).
	\end{equation}
	We know from Lemma~\ref{lem:bounding_constraints} that this sequence $a_i$ in~\eqref{eq:uglyai} satisfies the conditions from Lemma~\ref{lem:bounding}, so applyign Lemma~\ref{lem:bounding} one more time and combining all steps gives
	\begin{align*}
		\rho &= \sum_{i = 0}^{|D_u|}  p_i \left(\sum_{j = 0}^{|D_v|} \frac{1}{1+i+j}  q_j \right)\\
		& \geq \sum_{i = 0}^{|D_u|}  p_i \left( \frac{2}{9}\left( \frac{1}{i+1} + \frac{1}{i+3} \right) + \frac{5}{9} \left( \frac{1}{i+2} \right) \right) \\
		&\geq \frac{154}{405}.
	\end{align*}
	
	Therefore, we have shown in all possible subcases of Case 3 that $\prob\left[ \text{$e$ is satisfied} \mid X_u^c \cap X_v^c \right] \geq \frac{154}{405}$. 
	
	Cases 1,2, and 3 all together show that for every $e \in E$ we have
	\[
	\prob\left[ \text{$e$ is satisfied} \right] \geq \frac{154}{405} z_e.
	\]
\end{proof}

==> sections/hypergraphmaxecc.tex <==
Our hypergraph \maxecc{} approximation algorithm (Algorithm~\ref{alg:hyper_maxecc}) generates a uniform random priority for colors $\pi$, and independent random color thresholds $\{\alpha_c\}$ to determine which nodes want which colors. A node is then simply assigned to the highest priority color it wants. The proof of our approximation guarantee uses the following lemma, presented by~\citet{angel2016clustering} when developing the first approximation algorithm for graph \maxecc{}.
\begin{lemma}
	\label{lem:angel}
	Let $\left\{E_1, E_2, \dots, E_j \right\}$ be a set of independent events satisfying $\sum_{i=1}^j \prob[E_i] \leq 1$, then the probability that {at most one} of them happens is greater than or equal to $2/e$.
\end{lemma}
%Our new method satisfied the following result.
\begin{algorithm}[t]
    \caption{\textsf{HyperMaxECC}}
    \label{alg:hyper_maxecc}
    \begin{algorithmic}
        	\STATE Obtain optimal LP variables $\{z_e; x_v^c\}$ for the relaxation
        \STATE $\pi \leftarrow \text{uniform random ordering of colors } [k]$
        \STATE For $c \in [k]$, $\alpha_c \leftarrow $ uniform random threshold in $[0,1]$
        \FOR{$v \in V$}
        \STATE $W_v' = \{c \in [k] \colon \alpha_c < x_v^c\}$
        \IF{$|W_v'| > 0$}
        \STATE $\lambda(v) \leftarrow \argmax_{c \in W_v'} \pi(c)$
        \ELSE
        \STATE $\lambda(v) \leftarrow $ arbitrary color
        \ENDIF 
        \ENDFOR
    \end{algorithmic}
\end{algorithm}

\begin{theorem}
    Algorithm \ref{alg:hyper_maxecc} is a $\frac{1}{r+1} \left(\frac{2}{e}\right)^r$ approximation algorithm for \hypermaxecc{}.
\end{theorem}
\begin{proof}
Fix an arbitrary edge $e \in E$ with $c = \ell(e)$. Let $T_e$ denote the event that $e$ is satisfied. 
By Observation~\ref{obs:prob} it suffices to show $\prob[T_e] \geq \frac{1}{r+1} \left(\frac2e\right)^r$. 

Let $C = [k]\setminus \{c\}$ denote colors other than $c$. 
% For each $i \in C$, we would like quantify the possibility that some node in $e$ wants color $i$, as this opens up the possibility that $e$ will be dissatisfied because some node is given color $i$. Towards this goal, we identify a node in $e$ that has the highest likelihood of wanting $i$. Formally, for each color $i \in C$ we identify some node $v \in e$ satisfying $x_v^i \geq x_u^i$ for every $u \in e$ (breaking ties arbitrarily if multiple nodes satisfy this), and we define $\sigma(i) = v$. The definition of $\sigma(i)$ implies the following useful observation:
% \begin{observation}
% \label{obs:cv}
%     % One or more nodes in $e$ wants color $i$ if and only if $v = \sigma(i)$ wants color $i$. Equivalently, 
%     Color $i$ is not wanted by \textbf{any} nodes in $e$ $\iff$ color $i$ is not wanted by $v = \sigma(i)$.
% \end{observation}
To partition the color set $C$, for each $v \in e$ we define
\begin{equation*}
    C_v = \{i \in C \colon \sigma_e(i) = v\}
\end{equation*}
where we recall $\sigma_e(i)$ identifies a node $v \in e$ satisfying $x_v^i = \max_{u \in e} x_u^i$.
Let $A_v$ denote the event that at most one color in $C_v$ wants one or more nodes in $e$. From Observation~\ref{obs:cv}, $A_v$ is equivalent to the event that  $v$ wants at most 1 color in $C_v$. The probability of $A_v$ is therefore the probability that at most one of the events $\{X_v^i \colon i \in C_v \}$ happens. Combining Observation~\ref{obs:xuc} with the LP constraint $\sum_{i = 1}^k x_v^i = 1$ tells us that the assumptions of Lemma~\ref{lem:angel} hold, which in turn implies that $\prob[A_v] \geq 2/e$.
Observe now that the events $\{A_v \colon v \in e \}$ are mutually independent because the sets $\{C_v \colon v \in e\}$ are disjoint sets of colors, and the color thresholds $\{\alpha_i \colon i \in C\}$ are all drawn independently from each other. 

% To bound the probability of $T_e$ below, we will condition on the event that (i) every node in $e$ wants $c$ (i.e., event $Z_e$), and (ii) at most one color from each color set in $\{C_v \colon v \in e\}$ is wanted by one or more nodes in $e$ (i.e., $A_v$ holds for every $v \in e$). 
Since color thresholds are drawn independently for each color, we know the events $\{A_v, X_v^c \colon v \in e\}$ are all mutually independent.
%\footnote{For this independence argument to hold it is important that $c \notin C = [k] \backslash \{c\}$, meaning that nodes in $e$ wanting $c$ is not affected by which colors in $\{C_v \colon v \in e\}$ are wanted.}
Therefore, 
\begin{align*}
    \prob\left[ \left(\bigcap_{v \in e} A_v \right) \cap Z_e\right ] &= \prob[Z_e]\cdot \prod_{v \in e} \prob[A_v] \geq z_e \cdot \left(\frac2e \right)^r,
\end{align*}
where we have used Observation~\ref{obs:edgewants} and the independence of events. If both $Z_e$ and $\cap_{v \in e} A_v$ hold, this means that every node in $e$ wants color $c$, and at most $r$ distinct other colors (one for each node in $v \in e$ since there is one set $C_v$ for each $v \in e$) that want one or more nodes in $e$. Conditioned on this, in order for $e$ to be satisfied, the color $c$ must have a higher priority in the random ordering $\pi$ than the other $r$ colors, which happens with probability $1/(r+1)$. Putting this all together produces our needed probability bound:
\begin{align*}
    \prob[T_e] \geq \prob\left[T_e \mid Z_e \bigcap_{v \in e} A_v\right] \prob\left[ Z_e \bigcap_{v \in e} A_v \right] \geq \frac{z_e}{r+1}\left(\frac2e\right)^r.
\end{align*}


\end{proof}

==> sections/prelims.tex <==
\section{Preliminaries}
For a positive integer $n$, let $[n] = \{1,2, \hdots n\}$. 
We use bold lowercase letters to denote vectors, and indicate the $i$th of entry of a vector $\textbf{x} \in \mathbb{R}^n$ by $x_i$. For a set $S$ and a positive integer $t$, let ${S \choose t}$ denote all subsets of $S$ of size $t$.
An instance of edge-colored clustering is given by a hypergraph $H = (V,E, \ell)$ where $V$ is a node set, $E$ is a set of hyperedges (usually just called \emph{edges}), and $\ell \colon E \rightarrow [k]$ is a mapping from edges to a color set $[k] = \{1,2, \hdots, k\}$.  For $e \in E$, we let $\omega_e \geq 0 $ denote a nonnegative weight associated with $e$, which equals 1 for all edges in the unweighted version of the problem. For a color $c \in [k]$, let $E_c \subseteq E$ denote the edges of color $c$.

The goal of different variants of ECC is to construct a map $\lambda \colon V \rightarrow [k]$ that associates each node with a color. An edge $e \in E$ is \emph{satisfied} if $\ell(e) = \lambda(v)$ for every $v \in e$, and is otherwise \emph{unsatisfied}. The simplest variant is to color nodes to maximize the number of satisfied edges (\maxecc{}), which can be cast as the following binary linear program
\begin{align}
	\label{eq:maxecc}
\begin{aligned}
	\text{max} \quad& \textstyle \sum_{e \in E} \omega_e z_e \\
	\text{s.t.} \quad& \forall v \in V:\\
	&\forall c \in [k], e \in E_c:\\
	&x_v^c, z_e \in \{0, 1\}
\end{aligned}
\begin{aligned}
	&\\
	&\textstyle \sum_{c=1}^k x_v^c = 1 \\
	\quad &x_v^c \geq z_e \quad \forall v \in e \\
	&\forall c \in [k], v \in V, e \in E.
\end{aligned}
\end{align}
Setting $x_{u}^c$ to 1 indicates that node $u$ is given color $c$, i.e., $\lambda(u) = c$). We use $\textbf{x}_u = \begin{bmatrix} x_u^1 & x_u^2 & \cdots & x_u^k \end{bmatrix}$ to denote the vector of distances for node $u$. For edge $e \in E$, the constraints are designed in such a way that $z_e = 1$ if and only if $e$ is satisfied. A binary LP for \minecc{} can be obtained by changing the objective function above.
%but instead minimizing the objective $\sum_{e \in E} \omega_e (1 - z_e)$. 

%\textbf{Prior results on ECC.}
%Edge-colored clustering has been well-studied in the machine learning and data mining literature from the perspective of approximation algorithms~\cite{amburg2020clustering,amburg2022diverse,veldt2023optimal,crane2024overlapping,angel2016clustering} and fixed parameter tractability results~\cite{kellerhals2023parameterized,cai2018alternating,crane2024overlapping}. 
%The earliest work on edge-colored clustering focused on the \maxecc{} objective in graphs, proving a $1/e^2$ approximation algorithm by rounding a linear programming (LP) relaxation~\cite{angel2016clustering}, The rounding scheme was subsequently improved several times~\cite{ageev2015improved,alhamdan2019approximability} leading up to an approximation factor of 0.3622~\cite{ageev20200}.~\citet{amburg2020clustering} were the first to study the problem over hypergraphs, proving approximation algorithms for \minecc{}, which were later improved~\citet{veldt2023optimal}. Other variants of ECC include a regularized objective designed to create teams that are diverse and experienced with respect to past interaction types~\cite{amburg2022diverse}, and generalized ECC objectives that allow overlap in clusters~\cite{crane2024overlapping}. Several papers have also focused on fixed-parameter tractability results for different ECC objectives~\cite{cai2018alternating,kellerhals2023parameterized,crane2024overlapping}. 

%\textbf{Additional related work.}
%ECC is also closely related to chromatic correlation clustering (CCC)~\cite{bonchi2012chromatic,bonchi2015chromatic,anava2015improved,klodt2021color,xiu2022chromatic}, an edge-colored variant of correlation clustering~\cite{bansal2004correlation}. CCC can be viewed as variant of ECC in graphs in which one may have multiple clusters of the same color, and one additionally incurs penalties for clustering two nodes in the same colored cluster if they do not share an edge of that color. We note finally that our work on balanced and fair variants of ECC closely relates to other recent work on fair clustering and its applications, where the goal is to form cluster assignments that are in some sense balanced or proportional in terms of some class or feature within the data. We refer to the seminal work of \cite{chierichetti2017fair} and Section 5.3 of a recent survey~\cite{caton2024fairness} for more details. 
%As a final area of related work, our motivation to study balanced and fair variants of ECC closely relates to other recent work on fair clustering and its various applications, which has seen a , where the goal is to form cluster assignments that are in some sense balanced or proportional in terms of some class or feature within the data. We refer to the seminal work of \cite{chierichetti2017fair} and a recent survey 
